Local Discovery by Partitioning: Polynomial-Time Causal Discovery Around Exposure-Outcome Pairs

Causal discovery is crucial for causal inference in observational studies, as it can enable the identification of valid adjustment sets (VAS) for unbiased effect estimation. However, global causal discovery is notoriously hard in the nonparametric setting, with exponential time and sample complexity in the worst case. To address this, we propose local discovery by partitioning (LDP): a local causal discovery method that is tailored for downstream inference tasks without requiring parametric and pretreatment assumptions. LDP is a constraint-based procedure that returns a VAS for an exposure-outcome pair under latent confounding, given sufficient conditions. The total number of independence tests performed is worst-case quadratic with respect to the cardinality of the variable set. Asymptotic theoretical guarantees are numerically validated on synthetic graphs. Adjustment sets from LDP yield less biased and more precise average treatment effect estimates than baseline discovery algorithms, with LDP outperforming on confounder recall, runtime, and test count for VAS discovery. Notably, LDP ran at least 1300x faster than baselines on a benchmark.

==> definitions/definition_bias.tex <==
\begin{definition}
    \textbf{Bias in causal effect estimation.} We define bias as a systematic and nonrandom source of error in causal effect estimation \cite{holmberg_collider_2022}. Following \citet{hernan_causal_2020}, we present three dominant forms of bias:
    \begin{enumerate}[noitemsep,topsep=0pt]
        \item \textbf{Confounding bias.} Confounding is introduced by failing to control for variables that are common causes of both exposure and outcome. Confounding is among the most prominent problems facing valid causal inference under observational data \cite{hernan_causal_2020}. This form of bias prevents exchangeability between exposed and unexposed units, such that association and effect measures are not equal. Thus, ``association is not causation” even under infinite data when confounding is present \cite{hernan_causal_2020}. Confounding may arise from failure to adjust for common causes that are measured (syn. observed) or unmeasured (syn. latent, hidden, or unobserved). When confounding bias is eliminated, we can say that the causal relation is unconfounded.
        \item \textbf{Selection bias.} Like confounding, selection bias induces lack of exchangeability between exposed and unexposed units. Selection bias can arise in randomized and observational settings, as it is the product of study inclusion criteria \cite{hernan_causal_2020}. Controlling for a common effect of exposure and outcome, i.e. a collider, can introduce selection bias. This form of selection bias is often called collider bias \cite{holmberg_collider_2022}, and is a form of overadjustment \cite{lu_revisiting_2021}. Examples of selection bias in health research include Berkson's bias, differential loss to follow-up, non-response bias, and volunteer bias \cite{hernan_structural_2004}.
        \item \textbf{Measurement bias.} In practice, data are generally noisy and imperfectly measured. When the estimated association between exposure and outcome is influenced by the means of data collection, the study is said to suffer from measurement bias \cite{hernan_causal_2020}. Like selection bias, this can occur  under both randomized and observational study designs.
    \end{enumerate} \label{def:bias}
\end{definition}

==> definitions/definition_confounder.tex <==
\begin{definition}
    \textbf{Confounder.} For a variable $Z$ to be a confounder with respect to an exposure $X$ and an outcome $Y$, it must satisfy Property 1 and either Property 2 or Property 3, as defined by \citet{vanderweele_definition_2013}.
    \begin{enumerate}[noitemsep,topsep=0pt]
        \item \textbf{Property 1.} When $C$ is the set of all confounders for the effect of exposure $X$ on outcome $Y$, then all confounding bias has been eliminated from the effect of $X$ on $Y$ conditional on $C$. That is to say, $C$ meets the  definition of a sufficient adjustment set.
        \item \textbf{Property 2.} When $Z$ is a confounder for the effect of $X$ on $Y$, then there exists a set of pretreatment covariates $S$ of cardinality greater than or equal to zero such that $Y_x \ind X | (S \cup Z)$ but $Y_x \nind X | S$. That is to say, union with $Z$ is necessary for $S$ to constitute a sufficient adjustment set and thus to eliminate confounding bias.
        \item \textbf{Property 3.} When $Z$ is a confounder for the effect of $X$ on $Y$, there exists a set of pretreatment covariates $S$ of cardinality greater than or equal to zero such that
        \begin{align*}
            \left| \sum_{s,z}[\mathbb{E}(Y|X = 1,s,z) -  \mathbb{E}(Y|X = 0,s,z)] pr(s, z)  - [\mathbb{E}(Y_1)  -  \mathbb{E}(Y_0)] \right|&  < \\ 
            \left| \sum_s [\mathbb{E}(Y|X = 1,s) -  \mathbb{E}(Y|X = 0,s)] pr(s)  - [\mathbb{E}(Y_1)  -  \mathbb{E}(Y_0)] \right|&
        \end{align*}
        for the binary exposure setting, and analogously for continuous exposures. That is to say, adjusting for $Z$ in addition to $S$ reduces confounding bias relative to adjusting only for $S$. Note that this property is not scale invariant, e.g. $Z$ might be a confounder for $\{X,Y\}$ but not  $\{\log(X), \log(Y)\}$.
    \end{enumerate}

    Following from these properties, we take the definition of a confounder to be that given by \citet{vanderweele_definition_2013}: A confounder is a pretreatment covariate $Z$ for which there exists a set of covariates $S$ such that 1) $Z \notin S$ and $|S| \geq 0$, 2) the effect of exposure $X$ on outcome $Y$ is unconfounded conditional on $S \cup Z$, and 3) the effect of exposure on outcome is not unconfounded given any proper subset of $S \cup Z$.
    \label{def:confounder}
\end{definition}

==> definitions/definition_overadjustment.tex <==
\begin{definition}
\textbf{Overadjustment bias.} Broadly, overadjustment bias arises from adjustment for a variable that increases rather than decreases bias in effect estimation. Lu et al. (2021) delineate four types of overadjustment bias \cite{lu_revisiting_2021}:
\begin{enumerate}[noitemsep,topsep=0pt]
    \item \textbf{Type 1: Controlling for a mediator of the exposure and outcome (i.e. $\z_3$), or for a descendant of a mediator.} Adjusting for mediators results in null-biased total effect estimation \cite{schisterman_overadjustment_2009}, though such adjustment can enable controlled direct effect estimation under certain assumptions \cite{cole_fallibility_2002}. When the exposure has only an indirect effect on the outcome, the observed association between these variables conditional on the mediator(s) will be null in expectation. For the remainder of this paper, we refer to Type 1 overadjustment bias as mediator bias.
    \item \textbf{Type 2: Controlling for a collider of the exposure and outcome (i.e. $\z_2$), or for a descendant of a collider.} This form of bias is generally referred to as collider bias, and will be referred to as such for the remainder of this paper. As previously described, collider bias is a form of selection bias that undermines the internal validity of causal inferences \cite{holmberg_collider_2022}.
    \item \textbf{Type 3: Controlling for an instrumental variable (i.e. $\z_5$).} Let $Z$ be an instrument for exposure $X$ and outcome $Y$ such that changes in $Z$ directly induce changes in $X$ but only affect $Y$ indirectly, e.g. through the causal path $Z \rightarrow X \rightarrow Y$. When $X$ and $Y$ are latently confounded, controlling for $Z$ can amplify existing bias and reduce estimate precision \cite{lu_revisiting_2021}. Pearl notes that conditioning on instrumental variables can amplify existing confounding bias in both linear and nonlinear models, and can introduce new additional biases in nonlinear models \cite{pearl_class_2012}. Hereafter, we will refer to Type 3 bias as instrument bias.
    \item \textbf{Type 4: Controlling for a descendent of the outcome variable (i.e. $\z_6$) when exposure and outcome are causally related.} This form of bias produces a spurious association between exposure and outcome on the risk difference and risk ratio scales \cite{lu_revisiting_2021}. This can be viewed as a special case of collider bias, where the outcome is a common effect of the exposure and another variable \cite{lu_revisiting_2021}.
\end{enumerate} \label{def:overadjustment}
\end{definition}



==> definitions/definition_unnecessary_adjustment.tex <==
\begin{definition}
\textbf{Unnecessary adjustment.} Unnecessary adjustment is control for a variable that neither decreases nor increases bias but does introduce statistical problems, e.g. greater estimate variance. \citet{schisterman_overadjustment_2009} note four kinds of variables whose control constitutes unnecessary adjustment. We will subsequently refer to these as Types 1–4 of unnecessary adjustment:
\begin{enumerate}[noitemsep,topsep=0pt]
    \item \textbf{Type 1:} Variables external to the causal system of interest (i.e. $\z_8$).
    \item \textbf{Type 2:} Causes of the exposure with no additional causal relation to the exposure-outcome pair (i.e. $\z_5$).
    \item \textbf{Type 3:} Causes of the outcome with no additional causal relation to the exposure-outcome pair (i.e. $\z_4$).
    \item \textbf{Type 4:} Descendants of exposure with no additional causal relation to the exposure-outcome pair (i.e. $\z_7$).
\end{enumerate} \label{def:unnecessary}
\end{definition}

==> figure_tex/figure_comparison_ten_node.tex <==
\begin{figure}[!h]
    \centering
    %\fbox{$n = 10k$ \newline \includegraphics[width=0.45\textwidth]{figures/comparison_ten-node_10k.png}}
    %\fbox{$n = 50k$ \newline \includegraphics[width=0.45\textwidth]{figures/comparison_ten-node_50k.png}}
    \tikz
      \node[draw,align=center]
      {\textsc{Bernoulli $|$ Linear $|$ $n = 1k$}  \\ \includegraphics[width=0.45\textwidth]{figures/comparison_ten-node_1k.png}};
    \tikz
      \node[draw,align=center]
      {\textsc{Bernoulli $|$ Linear $|$ $n = 5k$} \\ \includegraphics[width=0.45\textwidth]{figures/comparison_ten-node_5k.png}}; \\
      %%
      \hspace{0.15mm}
      %%
    \tikz
      \node[draw,align=center]
      {\textsc{Bernoulli $|$ Linear $|$ $n = 10k$}  \\ \includegraphics[width=0.45\textwidth]{figures/comparison_ten-node_10k.png}};
    \tikz
      \node[draw,align=center]
      {\textsc{Bernoulli $|$ Linear $|$ $n = 50k$} \\ \includegraphics[width=0.45\textwidth]{figures/comparison_ten-node_50k.png}};
    \caption{Ground truth (\textbf{A}) and inference results for Algorithm \ref{alg:method} (\textbf{B}), PC Algorithm (\textbf{C}), and FCI (\textbf{D}) on the synthetic 10-node DAG (Figure \ref{fig:ten_node_dag}) with Bernoulli noise, linear causal mechanisms, $X$ as a direct cause of $Y$, and $n \in \{1k, 5k, 10k, 50k\}$ observations. Structural equations are reported in Table \ref{tab:sem_discrete}. Independence was determined using chi-square testing and $\alpha = 0.005$. %Edge types for each algorithm are defined in Table \ref{tab:edge_types}. 
    Unlike other baselines, Algorithm \ref{alg:method} correctly infers that only $Z_1$ is a confounder under all sample sizes. %Runtimes for Algorithm \ref{alg:method} were also substatially lower, reflecting the lower number of independence tests required. 
    %%
    PC Algorithm predicts that confounder sets are $\{Z_2, Z_3\}$, $\{Z_1\}$, $\{Z_1, Z_3\}$, and $\{Z_1\}$ for all members of the inferred Markov equivalence class (MEC) for $n = 1k$, $n = 5k$, $n = 10k$, and $n = 50k$, respectively. Additionally, some members of the MEC returned by PC predict $Z_2$ to be a confounder at $n \in \{5k,10k,50k\}$. 
    %%
    FCI predicts that confounder sets are $\{Z_2, Z_3\}$, $\{Z_1, Z_2\}$, $\{Z_1, Z_2, Z_3\}$, and $\{Z_1\}$ for all members of the inferred MEC for $n = 1k$, $n = 5k$, $n = 10k$, and $n = 50k$, respectively. }
    %%%
    %In theory, adjustment for $Z_2$ would be expected to induce selection bias when estimating the effect of $X$ on $Y$, while adjusting for $Z_3$ would null-bias total effect estimates.}
    \label{fig:compare_ten-node}
\end{figure}

\begin{table}[!h]
    \centering
    \begin{tabular}{l c c c}
        \toprule
        $n$ & \textsc{Algorithm \ref{alg:method}} & \textsc{PC Algorithm} & \textsc{Fast Causal Inference} \\
        \hline
        $1k$ & 0.030 & 0.359 & 0.741 \\
        $5k$ & 0.031 & 0.401 & 0.590 \\
        $10k$ & 0.045 & 0.419 & 0.753 \\
        $50k$ & 0.062 & 0.742 & 0.863 \\
        \bottomrule
    \end{tabular}
    \caption{Runtimes (in seconds) for obtaining the DAGs pictured in Figure \ref{fig:compare_ten-node}.}
    \label{tab:time_compare_ten-node}
\end{table}


==> figure_tex/figure_triples.tex <==
\begin{figure*}[H]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/triple.png}
    \caption{All potential acyclic triple subgraphs that can be induced by $X$, $Y$, and a single $Z$ when paths are restricted to a length of 1. The dashed arrow from $X$ to $Y$ indicates that the strength of this relation is unknown. %While the effect of $X$ on $Y$ might be null, it is known that $X \nind Y$ and that $Y$ does not cause $X$. The partition taxonomy proposed in this work (Table \ref{tab:partitions}) generalizes these cases to more complex structures. In the more complex setting, edges represent both direct adjacencies and indirect active paths. The absence of a directed edge therefore indicates either an inactive or nonexistent path.
    }
    \label{fig:triples}
\end{figure*}

%Kyra: the figure is way too small if we fit it into a single column

==> figure_tex/schematic.tex <==
\colorlet{Z1color}{WildStrawberry}
\colorlet{ZPOSTcolor}{YellowGreen}
\colorlet{Z4color}{OliveGreen}
\colorlet{Z5color}{TealBlue}
\colorlet{Z7color}{Melon}
\colorlet{Z8color}{Mulberry}

%https://tex.stackexchange.com/questions/651252/make-half-half-shaded-nodes-in-tikz
\tikzset{
  prefix after node/.style={prefix after command=\pgfextra{#1}},
  /semifill/ang/.initial=45,
  /semifill/upper/.initial=none,
  /semifill/lower/.initial=none,
  semifill/.style={
    circle, draw,
    prefix after node={
      \pgfqkeys{/semifill}{#1}
      \path let \p1 = (\tikzlastnode.north), \p2 = (\tikzlastnode.center),
                \n1 = {\y1-\y2} in [radius=\n1]
            (\tikzlastnode.\pgfkeysvalueof{/semifill/ang}) 
            edge[
              draw=none,
              fill=\pgfkeysvalueof{/semifill/upper},
              to path={
                arc[start angle=\pgfkeysvalueof{/semifill/ang}, delta angle=180]
                -- cycle}] ()
            (\tikzlastnode.\pgfkeysvalueof{/semifill/ang}) 
            edge[
              draw=none,
              fill=\pgfkeysvalueof{/semifill/lower},
              to path={
                arc[start angle=\pgfkeysvalueof{/semifill/ang}, delta angle=-180]
                -- cycle}] ();}}}

\begin{table}[!h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{|c|c|c|c|}
    \hline
    & & & \\
    \input{figure_tex/schematic_step_0} & \input{figure_tex/schematic_step_1} & \input{figure_tex/schematic_step_2} & \input{figure_tex/schematic_step_3} \\
    \hline
    & & & \\
    \input{figure_tex/schematic_step_4} & \input{figure_tex/schematic_step_5} & \input{figure_tex/schematic_step_6} & \input{figure_tex/schematic_step_7} \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \vspace{2mm}
    \caption{Schematic of Algorithm \ref{alg:method}. The exposure-outcome pair $\{X,Y\}$ serves as a nucleus around which LDP assembles a partial causal graph. Each step reveals additional information about the partitions of $\z$. Nodes that are fully colored are fully discovered by Algorithm \ref{alg:method}. Partial coloring denotes partial knowledge, and no coloring denotes no knowledge.}
    \label{tab:schematic}
\end{table}

Table \ref{tab:schematic} provides a visual walk-through of Algorithm \ref{alg:method} as knowledge is progressively obtained at each step. In plain English, the steps of Algorithm \ref{alg:method} are as follows.

\begin{enumerate}[noitemsep,topsep=0pt,label={\itshape Step \arabic*},leftmargin=\widthof{[Step 7]}+\labelsep]%align= left]
    \item $\z_8$ is discovered using prior knowledge of $\{X,Y\}$ only. 
    \item $\z_4$ is discovered using prior knowledge of $\{X,Y\}$ only. 
    \item  $\z_{7}$ is discovered using prior knowledge of $\{X,Y\}$ only. Some or all of $\z_5$ can also be discovered at this step for some graphical structures (e.g., when $|\z_1| = 0$). %In practice, we have occasionally observed this happening under small finite samples even when $|\z_1| > 0$.  
    \item A fraction of $\z_{\textsc{Post}}$ is discovered, providing complete knowledge of $\z_6$ and partial knowledge of $\z_2$ and $\z_3$. This step leverages prior knowledge of $\z_4$ that was obtained programmatically at Step 2. 
    \item $\z_{\textsc{Mix}}$ is temporarily aggregated, providing partial knowledge of $\z_1$, $\z_2$, $\z_3$, and $\z_5$. $\z_{\textsc{Mix}}$ is a transient superset that is used to  differentiate $\z_1$ and $\z_5$ from $\z_{\textsc{Post}}$ in Step 6. The partitions that can be represented in $\z_{\textsc{Mix}}$ will depend on whether sufficient condition \ref{cond:sufficient_1} is violated or not.
    \item Knowledge of $\z_{\textsc{Post}}$ is complete. $\z_{\textsc{Mix}}$ is fully disaggregated, providing final partition labels for a fraction of members and moving others to superset $\z_{1,5}$. In the process, a fraction of $\z_1$ is placed in $\z_1$. %A fraction of $\z_1$ and $\z_5$ may still be indistinguishable from each other. 
    At this step, we union the  $\z_{\textsc{Mix}}$ discovered in Step 5 with the $\z_{5,7}$ discovered at Step 3. This is under the assumption that some $\z_5$ might have been discovered at Step 3, and will need to be distinguished from $\z_7$. Thus, this step serves as a final check on the set-purity of $\z_7$, and knowledge of $\z_7$ is complete.
    \item $\z_1$ and $\z_5$ are fully differentiated from each other. This step tests whether a member of the superset $\z_{1,5}$ is marginally dependent on any known $Z_1$. All previously known $Z_1$ are those that are directly adjacent to $Y$. $Z_1$ that are left to be discovered are those with indirect active paths to $Y$. Even when sufficient condition \ref{cond:sufficient_1} is violated, no $Z_5$ will ever be dependent on a $Z_1$ that is directly adjacent to $Y$. However, all $Z_1$ will be marginally dependent on at least one $Z_1$ that is adjacent to $Y$. 
\end{enumerate}


==> tables_tex/table_benchmarks.tex <==
\begin{table}[!h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l cccc cccc cccc}
        \toprule
        %%%
         &  \multicolumn{4}{c}{\fontfamily{cmr}\textsc{\textbf{Barley}}  \textsc{aks\_m2} $\to$ \textsc{keraks}} &  \multicolumn{4}{c}{\fontfamily{cmr}\textsc{\textbf{Mildew}}  \textsc{mikro\_1} $\to$ \textsc{meldug\_2} ($d = 16$)} & \multicolumn{4}{c}{\fontfamily{cmr}\textsc{\textbf{Hailfinder}} \textsc{area} $\to$ \textsc{clds}}  \\ 
         %%%
         \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
         %%%
         $n$ & $\z$ \textsc{Acc} & $\z_1$ \textsc{Pre} & $\z_1$ \textsc{Rec} & \cmark & $\z$ \textsc{Acc} & $\z_1$ \textsc{Pre} & $\z_1$ \textsc{Rec} & \cmark & $\z$ \textsc{Acc} & $\z_1$ \textsc{Pre} & $\z_1$ \textsc{Rec} & \cmark \\
         %%%
         \hline
         %%%
         $10k$ & x & x & x & x & 71.4 (53.2-89.7) & 53.3 (9.0-97.6) & 60.0 (12.0-100) & 2/5 & x & x  & x & x \\
         $25k$ & x & x & x & x & 88.6 (76.4-100) & 80.0 (40.8-100) & 80.0 (40.8-100) & 4/5 & x  & x & x & x \\
         $50k$ & x & x & x & x & 92.9 (92.9-92.9) & 100 (100-100) & 100 (100-100) & 5/5 & x  & x & x & x \\
         $100k$ & x & x & x & x & 92.9 (88.4-97.3) & 100 (100-100) & 100 (100-100) & 5/5 & x  & x & x & x \\
         %$250k$ & x & x & x & x & x & x & x & x & x  & x & x & x \\
         %%%%%%%%%%%%%%%%%%%
         %% MILDEW
         %%%%%%%%%%%%%%%%%%%
         %\toprule
         %& \multicolumn{4}{c}{\fontfamily{cmr}\textsc{\textbf{Mildew}}  \textsc{mikro\_1} $\to$ \textsc{meldug\_2}} \\
         %%%%%%%%%%%%%%%%%%%
         %% ?
         %%%%%%%%%%%%%%%%%%%
         %& \multicolumn{4}{c}{\fontfamily{cmr}\textsc{\textbf{Hailfinder}} \textsc{area} $\to$ \textsc{clds}}  \\
         \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Performance of Algorithm \ref{alg:method} on discrete benchmark data from \texttt{bnlearn} \citep{scutari_learning_2010}. Sample size is denoted by $n$ and dimensionality by $d$ (including exposure and outcome). Exposure $X$ and outcome $Y$ are denoted by $X \to Y$. All values are averaged over five independent data samples from the underlying DAG. Metrics reported are accuracy of all labels ($\z$ \textsc{Acc}), precision for partition $\z_1$ ($\z_1$ \textsc{Pre}), recall for partition $\z_1$ ($\z_1$ \textsc{Rec}), and fraction of replicates that admit a sufficient adjustment set (\cmark). Standard deviations are in parentheses. The 95\% confidence interval over the 100 individual DAG metrics is reported in parentheses. Independence was determined by permutation testing with 20 permutation surrogates for $n = 100k$, 30 surrogates for $n = 50k$, and 50 surrogates for $n < 50k$.}
    \label{tab:benchmarks}
\end{table}

==> tables_tex/table_benchmarks_old.tex <==
\begin{table*}[!h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l | ccc ccc ccc | ccc ccc ccc}
    \toprule[1pt]
        & \multicolumn{9}{c}{\fontfamily{cmr}\textsc{\textbf{Lung}} ($d = 8$, $d' = 8$) $|$ \textsc{either} $\to$ \textsc{dysp}} &  \multicolumn{9}{|c}{\fontfamily{cmr}\textsc{\textbf{Barley}} ($d = 48$, $d' = 7$) $|$ \textsc{jordinf} $\to$ \textsc{markgm}}  \\
        %%%
        \cmidrule(lr){2-10} \cmidrule(lr){11-19} 
        %%%
         & \multicolumn{3}{c}{\textsc{Heuristic}} & \multicolumn{3}{c}{\textsc{Random}} & \multicolumn{3}{c}{\textsc{Restricted}} & \multicolumn{2}{|c}{\textsc{Heuristic}} & \multicolumn{3}{c}{\textsc{Random}} & \multicolumn{3}{c}{\textsc{Restricted}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
        %%%
        $n$ & $\z$ & $\z_1$ & \cmark  & $\z$ & $\z_1$ & \cmark  & $\z$ & $\z_1$ & \cmark  & $\z$ & $\z_1$ & \cmark  & $\z$ & $\z_1$ & \cmark  & $\z$ & $\z_1$ & \cmark  \\
        %%%
        \hline
        $50k$ & & & &  &  &  \\
        $100k$ & 100.0 & 100.0 & \cmark & 83.33 & 83.33 & \cmark & 66.67 & 66.67 & \xmark & 100.0 & 100.0 & \cmark & 85.71 & 100.0 & \cmark & 100.0 & 100.0 & \cmark  \\
        %%%%%%%%
        %%%%%%%%
        %%%%%%%%
        \toprule[1pt]
        & \multicolumn{9}{c}{\fontfamily{cmr}\textsc{\textbf{Mildew}} ($d = 35$, $d' = 10$) $|$ \textsc{mikro\_1} $\to$ \textsc{meldug\_2}} & \multicolumn{9}{|c}{\fontfamily{cmr}\textsc{\textbf{Barley}} ($d = 48$, $d' = 10$) $|$ \textsc{aks_m2} $\to$ \textsc{keraks} }  \\
        %%%
        \cmidrule(lr){2-10} \cmidrule(lr){11-19} 
        %%%
         & \multicolumn{3}{c}{\textsc{Heuristic}} & \multicolumn{3}{c}{\textsc{Random}} & \multicolumn{3}{c}{\textsc{Restricted}} & \multicolumn{2}{|c}{\textsc{Heuristic}} & \multicolumn{3}{c}{\textsc{Random}} & \multicolumn{3}{c}{\textsc{Restricted}} \\
        %%%
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
        %%%
        $n$ & $\z$ & $\z_1$ & \cmark & $\z$ & $\z_1$ & \cmark  & $\z$ & $\z_1$ & \cmark  & $\z$ & $\z_1$ & \cmark  & $\z$ & $\z_1$ & \cmark  & $\z$ & $\z_1$ & \cmark  \\
        %%%
        \hline
        $50k$ &  &  &  &  &  &  \\
        $100k$ & 90.0 (0) & 100.0 (0) & 5/5 & 88.0 (4.0) & 90.0 & 3/5 & 80.0 & 90.0 &    \\
        %%%%%%%%
    \toprule[1pt]
    \end{tabular}
    \end{adjustbox}
    \caption{Accuracy of Algorithm \ref{alg:method} on discrete benchmark data from \texttt{bnlearn}. Sample size is denoted by $n$, total variables in the ground truth DAG by $d$, and total variables tested using Algorithm \ref{alg:method} by $d'$. Exposure $X$ and outcome $Y$ are denoted by $X \to Y$. All values are averaged over five independent data samples from the underlying DAG. Accuracies are reported as percent of total labels that are correct ($\z$), percent of correct binary labels \textit{confounder} vs \textit{not confounder} ($\z_1$), and fraction of replicates that admit a sufficient adjustment set (\cmark). Standard deviations are in parentheses. Three thresholding methods were used for determining statistical independence: manual selection (\textsc{Heuristic}), permutation testing with random shuffling of 10 surrogates ($\alpha = 0.1$) (\textsc{Random}), and permutation with restricted shuffling, as described by \citet{runge_conditional_2018} (\textsc{Restricted}).}
    \label{tab:benchmarks}
\end{table*}

==> tables_tex/table_bias_cases.tex <==
%\begin{itemize}[noitemsep,topsep=0pt]
    %\item $\z_2$: Type 2 overadjustment bias, i.e. collider bias.
    %\item $\z_3$: Type 1 overadjustment bias, i.e. mediator bias.
    %\item $\z_4$: Type 3 unnecessary adjustment.
    %\item $\z_5$: Type 2 unnecessary adjustment or Type 3 overadjustment bias, i.e. instrument bias.
    %\item $\z_6$: Type 4 overadjustment bias when $X$ causes $Y$.
    %\item $\z_7$: Type 4 unnecessary adjustment.
    %\item $\z_8$: Type 1 unnecessary adjustment.
%\end{itemize}
\begin{table}[!h]
    \centering
    %\begin{adjustbox}{max width=0.47\textwidth}
    %\begin{tabular}{p{0.5cm}|p{7cm}}
    \begin{tabular}{c | l}
    \toprule
        $\z_2$ & Type 2 overadjustment bias, i.e. collider bias. \\
        $\z_3$ & Type 1 overadjustment bias, i.e. mediator bias. \\
        $\z_4$ & Type 3 unnecessary adjustment. \\
        $\z_5$ & Type 2 unnecessary adjustment or Type 3 overadjustment bias, i.e. instrument bias. \\
        $\z_6$ & Type 4 overadjustment bias when $X$ causes $Y$. \\
        $\z_7$ & Type 4 unnecessary adjustment. \\
        $\z_8$ & Type 1 unnecessary adjustment. \\
    \bottomrule
    \end{tabular}
    %\end{adjustbox}
    \caption{Forms of bias introduced per variable case if that case were included in the final adjustment set, as defined by \citet{lu_revisiting_2021} and \citet{schisterman_overadjustment_2009} (Definitions \ref{def:overadjustment} and \ref{def:unnecessary}).}
    \label{tab:bias_cases}
\end{table}

==> tables_tex/table_bnlearn_barley.tex <==
\begin{table}[!h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l cccc cccc cccc}
        \toprule[1pt]
        %%%
        &  \multicolumn{12}{c}{\fontfamily{cmr}\textsc{\textbf{Barley}}  \textsc{aks\_m2} $\to$ \textsc{keraks} ($|\z| = 46$, $|\z_1| = 12$)} \\
        \cmidrule(lr){2-13}
        %%%
         &  \multicolumn{4}{c}{\textsc{Algorithm \ref{alg:method}}} &  \multicolumn{4}{c}{\textsc{PC}} & \multicolumn{4}{c}{\textsc{FCI}}  \\ 
         %%%
         \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
         %%%
         $n$ & $\z$ \textsc{Acc} & $\z_1$ \textsc{Pre} & $\z_1$ \textsc{Rec} & \cmark & $\z$ \textsc{Acc} & $\z_1$ \textsc{Pre} & $\z_1$ \textsc{Rec} & \cmark & $\z$ \textsc{Acc} & $\z_1$ \textsc{Pre} & $\z_1$ \textsc{Rec} & \cmark \\
         %%%
         \hline
         %%%
         $10k$ & 60.0 (48.6-71.4) & 93.5 (88.1-98.8) & 58.3 (42.0-74.7) & x & x & x & x & x & x & x  & x & x \\
         $25k$ & 84.3 (76.1-92.4) & 94.8 (90.6-99.0) & 86.7 (76.9-96.5) & x & x & x & x & x & x & x  & x & x \\
         $50k$ & 85.7 (85.7-85.7) & 93.5 (90.2-96.7) & 91.7 (86.5-96.8) & x & x & x & x & x & x & x  & x & x \\
         %$100k$ & x & x & x & x & x & x & x & x & x & x  & x & x \\
         %%%
         \bottomrule[1pt]
    \end{tabular}
    \end{adjustbox}
    \caption{Performance of Algorithm \ref{alg:method} on the \textsc{Barley} benchmark from \texttt{bnlearn} \citep{scutari_learning_2010}, with \textsc{aks\_m2} as exposure and \textsc{keraks} as outcome. All values are averaged over five independent data samples from the ground truth DAG, with 95\% confidence intervals in parentheses. Sample size is denoted by $n$. All 48 variables in the original DAG were submitted to Algorithm \ref{alg:method} with a chi-square independence test ($\alpha = 0.005$). An arbitrary 14-node subset meeting the assumptions of Algorithm \ref{alg:method} was assigned manual labels as ground truth, which were used to assess predicted label quality. Metrics reported are mean accuracy of all labels ($\z$ \textsc{Acc}), mean precision for partition $\z_1$ ($\z_1$ \textsc{Pre}), mean recall for partition $\z_1$ ($\z_1$ \textsc{Rec}), and fraction of replicates that admit a sufficient adjustment set (\cmark). }
    \label{tab:barley}
\end{table}

==> tables_tex/table_forbidden.tex <==
\newcommand{\tikzxmark}{%
\tikz[scale=0.23] {
    \draw[line width=1,line cap=round] (0,0) to [bend left=6] (1,1);
    \draw[line width=1,line cap=round] (0.2,0.95) to [bend right=3] (0.8,0.05);
}}


\setlength{\tabcolsep}{0.3em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.3} % for the vertical padding

\setlength{\fboxrule}{0.75pt}
\begin{figure}[!h]
    \centering
    \fbox{\begin{adjustbox}{max width=0.22\textwidth}
    \begin{tabular}{c | c c c c c c c c}
    %\toprule[1pt]
    \multicolumn{9}{c}{\textsc{any type of active path}} \\
    \toprule
         & $\z_1$ & $\z_2$ & $\z_3$ & $\z_4$ & $\z_5$ & $\z_6$ & $\z_7$ & $\z_8$ \\
         \hline
         $\z_1$ & \cmark & & &  &  &  &  &  \\
         $\z_2$ & \cmark & \cmark &  & &  & &  &  \\
         $\z_3$ & \cmark & \cmark & \cmark &  &  & &  &  \\
         $\z_4$ & \cmark & \cmark & \cmark & \cmark &  & &  &  \\
         $\z_5$ & \cmark & \cmark & \xmark & \xmark & \cmark &  & &  \\
         $\z_6 $& \xmark & \cmark & \xmark & \cmark & \xmark & \cmark &  &  \\
         $\z_7$ & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark &  \\
         $\z_8$ & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \cmark\\
    %\bottomrule[1pt]
    \end{tabular}
    \end{adjustbox}}
    %%%%%%%%%%%%
    %\hspace{0.1mm}
    %%%%%%%%%%%%
    \fbox{\begin{adjustbox}{max width=0.22\textwidth}
    \begin{tabular}{c | c c c c c c c c}
    %\toprule[1pt]
    \multicolumn{9}{c}{$Z_{row} \rightarrow \dots \rightarrow Z_{col}$} \\
    \toprule
         & $\z_1$ & $\z_2$ & $\z_3$ & $\z_4$ & $\z_5$ & $\z_6$ & $\z_7$ & $\z_8$ \\
         \hline
         $\z_1$ & \cmark &  & &  &  &  &  &  \\
         $\z_2$ & \xmark & \cmark & &  &  &  &  &  \\
         $\z_3$ & \cmark & \cmark & \cmark &  &  &  &  &  \\
         $\z_4$ & \xmark & \cmark & \cmark & \cmark &  &  &  &  \\
         $\z_5$ & \xmark & \cmark & \xmark & \xmark & \cmark &  &  &  \\
         $\z_6$ & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark &  &  \\
         $\z_7$ & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark &  \\
         $\z_8$ & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \cmark \\
    %\bottomrule[1pt]
    \end{tabular}
    \end{adjustbox}}
    %%%%
    %\hspace{0.1mm}
    %%%%
    \fbox{\begin{adjustbox}{max width=0.22\textwidth}
    \begin{tabular}{c | c c c c c c c c}
    %\toprule[1pt]
    \multicolumn{9}{c}{$Z_{row} \leftarrow \dots \leftarrow Z_{col}$} \\
    \toprule
         & $\z_1$ & $\z_2$ & $\z_3$ & $\z_4$ & $\z_5$ & $\z_6$ & $\z_7$ & $\z_8$ \\
         \hline
         $\z_1$ & \cmark &  & &  &  &  &  &  \\
         $\z_2$ & \cmark & \cmark & &  &  &  &  &  \\
         $\z_3$ & \cmark & \xmark & \cmark &  &  &  &  &  \\
         $\z_4$ & \xmark & \xmark & \xmark & \cmark &  &  &  &  \\
         $\z_5$ & \xmark & \xmark & \xmark & \xmark & \cmark &  &  &  \\
         $\z_6$ & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark &  &  \\
         $\z_7$ & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \cmark &  \\
         $\z_8$ & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark  & \cmark \\
    %\bottomrule[1pt]
    \end{tabular}
    \end{adjustbox}}
    %%%%
    %\hspace{0.1mm}
    %%%%
    \fbox{\begin{adjustbox}{max width=0.22\textwidth}
    \begin{tabular}{c | c c c c c c c c}
    %\toprule[1pt]
    \multicolumn{9}{c}{$Z_{row} \leftarrow \dots Z' \dots \rightarrow Z_{col}$} \\
    \toprule
         & $\z_1$ & $\z_2$ & $\z_3$ & $\z_4$ & $\z_5$ & $\z_6$ & $\z_7$ & $\z_8$ \\
         \hline
         $\z_1$ & \cmark & & &  &  &  &  &  \\
         $\z_2$ & \cmark & \cmark & &  &  &  &  &  \\
         $\z_3$ & \cmark & \cmark & \cmark &  &  &  &  &  \\
         $\z_4$ & \xmark & \cmark & \cmark & \cmark &  &  &  &  \\
         $\z_5$ & \xmark & \cmark & \xmark & \xmark & \cmark &  &  &  \\
         $\z_6$ & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark &  &  \\
         $\z_7$ & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark &  \\
         $\z_8$ & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark  & \cmark \\
    %\bottomrule[1pt]
    \end{tabular}
    \end{adjustbox}}
    \caption{Subsets of $\z$ that can and cannot share active paths with each other, following from the definition of each variable type (Table \ref{tab:partitions}). The symbol \xmark \, indicates that the given subset pair cannot share an active path of the designated type (under Definition \ref{def:path_types}) without violating the definitions of these subsets or some graphical assumption, e.g. acyclicity. The symbol \cmark \, indicates that the given  pair can share at least one active path of the designated type.}
    \label{fig:forbidden}
\end{figure}

==> tables_tex/table_latent_pretreatment.tex <==
\begin{table}[!h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l c c c c c c}
    \toprule
    & \multicolumn{3}{c}{\textsc{Figure \ref{fig:latent_experiments} (left)}} & \multicolumn{3}{c}{\textsc{Figure \ref{fig:latent_experiments} (right)}} \\
    %\cmidrule(lr){2–4}  \cmidrule(lr){5–7} 
    %%%%
    \textsc{Latent Confounder} & None & $Z_{5a}$ & $Z_{4a}$ & None & $Z_{5b}$ & $Z_{4b}$ \\
    \midrule
    \textsc{Label Accuracy} & 98.2 (97.7–98.7) & 100 (100–100) & 100 (100–100) & 100 (100–100) & 100 (100–100) & 100 (100–100) \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Performance of LDP for causally insufficient linear–Gaussian DAGs (Figure \ref{fig:latent_experiments}) with pretreatment $\z$ numerically validates Theorem \ref{theorem:pretreatment_latents}. Label accuracy is computed with the expected label for LDP under causal sufficiency as the ground truth. This is to accommodate the fact that LDP is \textit{expected} to mislabel $Z_{1a}$ and $Z_{1c}$ as $\z_{\textsc{Post}}$ even when there are no latent variables in $\g$, though the returned $\z_1$ ($\{Z_{1b}\}$) is still expected to be a valid adjustment set. All other variables in Figure \ref{fig:latent_experiments} are expected to have correct partition labels. Accuracies are averaged over 100 replicate DAGs with identical structure and varying coefficients, with structural equations reported in Table \ref{tab:sem_continuous}. The 95\% confidence intervals are reported in parentheses. Independence is determined by Fisher-z tests ($\alpha = 0.005$). All experiments were run on a 2017 MacBook with 2.9 GHz Quad-Core Intel Core i7.}
    \label{tab:latent_pretreatment}
\end{table}

==> tables_tex/table_m_butterfly_latent.tex <==
\begin{table}[!h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l ccc ccc}
    \toprule
%%%%%%%%%%%%%%%%%%%%%
%% All observed
%%%%%%%%%%%%%%%%%%%%%
    & \multicolumn{6}{c}{\fontfamily{cmr}\textsc{\textbf{All Variables Observed}}} \\
    \cmidrule(lr){2-7} 
    %%%
     & \multicolumn{3}{c}{\textsc{Bernoulli $|$ Linear}} & \multicolumn{3}{c}{\textsc{Hypergeometric $|$ Quadratic}} \\
     \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
     %%%
$n$ & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} \\
\hline
$500$ & 73.5 (71.0-76.0) & 26.2 (17.6-34.9) & 27.0 (18.3-35.7) & 75.3 (73.8-76.8) & 16.0 (8.8-23.2) & 16.0 (8.8-23.2) \\
$1k$ & 92.1 (90.4-93.8) & 90.0 (84.1-95.9) & 90.0 (84.1-95.9) & 87.3 (85.8-88.7) & 94.0 (89.3-98.7) & 94.0 (89.3-98.7) \\
$5k$ & 97.1 (96.0-98.2) & 97.0 (93.6-100) & 97.0 (93.6-100) & 99.8 (99.6-100) & 100 (100-100) & 100 (100-100) \\
$10k$ & 99.7 (99.4-100) & 100 (100-100) & 100 (100-100) & 100 (100-100) & 100 (100-100) & 100 (100-100) \\
%%%%%%%%%%%%%%%%%%%
         \toprule
%%%%%%%%%%%%%%%%%%%%%
%% M1 dropped
%%%%%%%%%%%%%%%%%%%%%
    & \multicolumn{6}{c}{\fontfamily{cmr}\textsc{\textbf{$M_1$ Unobserved}}} \\
    \cmidrule(lr){2-7} 
    %%%
     & \multicolumn{3}{c}{\textsc{Bernoulli $|$ Linear}} & \multicolumn{3}{c}{\textsc{Hypergeometric $|$ Quadratic}} \\
     \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
     %%%
$n$ & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} \\
\hline
$500$ & 69.2 (66.4-72.0) & 17.0 (9.6-24.4) & 17.0 (9.6-24.4) & 72.8 (71.3-74.3) & 13.0 (6.4-19.6) & 13.0 (6.4-19.6) \\
$1k$ & 92.4 (90.5-94.3) & 69.0 (59.9-78.1) & 69.0 (59.9-78.1) & 90.4 (88.8-92.0) & 83.0 (75.6-90.4) & 83.0 (75.6-90.4) \\
$5k$ & 96.0 (94.4-97.6) & 80.0 (72.1-87.9) & 80.0 (72.1-87.9) & 100 (100-100) & 100 (100-100) & 100 (100-100) \\
$10k$ & 99.8 (99.4-100) & 99.0 (97.0-100) & 99.0 (97.0-100) & 99.8 (99.4-100) & 99.0 (97.0-100) & 99.0 (97.0-100) \\
%%%%%%%%%%%%%%%%%%%
             \toprule
%%%%%%%%%%%%%%%%%%%%%
%% M2 dropped
%%%%%%%%%%%%%%%%%%%%%
    & \multicolumn{6}{c}{\fontfamily{cmr}\textsc{\textbf{$M_2$ Unobserved}}} \\
    \cmidrule(lr){2-7} 
    %%%
     & \multicolumn{3}{c}{\textsc{Bernoulli $|$ Linear}} & \multicolumn{3}{c}{\textsc{Hypergeometric $|$ Quadratic}} \\
     \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
     %%%
$n$ & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} \\
\hline
$500$ & 57.4 (53.5-61.3) & 27.0 (18.3-35.7) & 27.0 (18.3-35.7) & 76.8 (74.5-79.1) & 37.0 (27.6-46.4) & 39.0 (29.4-48.6) \\
$1k$ & 84.6 (83.3-85.9) & 92.8 (87.9-97.7) & 94.0 (89.3-98.7) & 87.8 (86.3-89.3) & 98.0 (95.2-100) & 98.0 (95.2-100) \\
$5k$ & 78.1 (77.0-79.2) & 30.3 (28.5-32.2) & 91.0 (85.4-96.6) & 79.8 (79.5-80.1) & 34.0 (33.4-34.6) & 100 (100-100) \\
$10k$ & 80.0 (80.0-80.0) & 33.3 (33.3-33.3) & 100 (100-100) & 80.0 (80.0-80.0) & 33.3 (33.3-33.3) & 100 (100-100) \\
%%%%%%%%%%%%%%%%%%%
                  \toprule
%%%%%%%%%%%%%%%%%%%%%
%% M3 dropped
%%%%%%%%%%%%%%%%%%%%%
    & \multicolumn{6}{c}{\fontfamily{cmr}\textsc{\textbf{$M_3$ Unobserved}}} \\
    \cmidrule(lr){2-7} 
    %%%
     & \multicolumn{3}{c}{\textsc{Bernoulli $|$ Linear}} & \multicolumn{3}{c}{\textsc{Hypergeometric $|$ Quadratic}} \\
     \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
     %%%
$n$ & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} \\
\hline
$500$ & 78.1 (75.9-80.3) & 19.0 (11.3-26.7) & 19.0 (11.3-26.7) & 82.0 (80.7-83.3) & 11.0 (4.8-17.2) & 11.0 (4.8-17.2) \\
$1k$ & 94.2 (92.8-95.6) & 96.0 (92.1-99.9) & 96.0 (92.1-99.9) & 91.1 (89.3-92.9) & 86.0 (79.2-92.8) & 86.0 (79.2-92.8) \\
$5k$ & 97.7 (96.7-98.7) & 99.0 (97.0-100) & 99.0 (97.0-100) & 99.9 (99.7-100) & 100 (100-100) & 100 (100-100) \\
$10k$ & 99.9 (99.7-100) & 99.5 (98.5-100) & 100 (100-100) & 99.7 (99.4-100) & 100 (100-100) & 100 (100-100) \\
%%%%%%%%%%%%%%%%%%%
                 \toprule
%%%%%%%%%%%%%%%%%%%%%
%% M1 and M2 dropped
%%%%%%%%%%%%%%%%%%%%%
    & \multicolumn{6}{c}{\fontfamily{cmr}\textsc{\textbf{$M_1$ and $M_2$ Unobserved}}} \\
    \cmidrule(lr){2-7} 
    %%%
     & \multicolumn{3}{c}{\textsc{Bernoulli $|$ Linear}} & \multicolumn{3}{c}{\textsc{Hypergeometric $|$ Quadratic}} \\
     \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
     %%%
$n$ & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} \\
\hline
$500$ & 65.8 (61.9-69.7) & 23.0 (14.7-31.3) & 23.0 (14.7-31.3) & 74.6 (72.3-76.8) & 35.0 (25.6-44.4) & 35.0 (25.6-44.4) \\
$1k$ & 91.9 (89.9-93.8) & 70.5 (61.9-79.1) & 74.0 (65.4-82.6) & 89.1 (87.4-90.9) & 90.0 (84.1-95.9) & 90.0 (84.1-95.9) \\
$5k$ & 66.7 (66.7-66.7) & 0.0 (0.0-0.0) & 0.0 (0.0-0.0) & 66.7 (66.7-66.7) & 0.0 (0.0-0.0) & 0.0 (0.0-0.0) \\
$10k$ & 66.7 (66.7-66.7) & 0.0 (0.0-0.0) & 0.0 (0.0-0.0) & 66.9 (66.2-67.6) & 1.0 (0-3.0) & 1.0 (0-3.0) \\
     %%%%%%%%%%%%%%%%%%%
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Performance of Algorithm \ref{alg:method} on thirteen-node DAGs containing an M-structure structure (Figure \ref{fig:m_butterfly}) across noise distributions, causal mechanisms, and sample sizes ($n$). In all DAGs, exposure $X$ is a direct cause of outcome $Y$. Metrics reported are accuracy of all labels ($\z$ \textsc{Acc}), mean precision for partition $\z_1$ ($\z_1$ \textsc{Pre}), and mean recall for partition $\z_1$ ($\z_1$ \textsc{Rec}). The 95\% confidence interval over the 100 individual DAG metrics is reported in parentheses. Independence was determined by chi-square independence testing with $\alpha = 0.001$.} 
    \label{tab:results_m}
\end{table}


\begin{table}[!h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l ccc ccc}
    \toprule
%%%%%%%%%%%%%%%%%%%%%
%% All observed
%%%%%%%%%%%%%%%%%%%%%
          & \multicolumn{6}{c}{\fontfamily{cmr}\textsc{\textbf{All Variables Observed}}} \\
         \cmidrule(lr){2-7} 
         %%%
         & \multicolumn{3}{c}{\textsc{Bernoulli $|$ Linear}} & \multicolumn{3}{c}{\textsc{Hypergeometric $|$ Quadratic}} \\
         \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
          %%%
         $n$ & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} \\
         %%%
         \hline
$1k$ & 60.4 (57.5-63.2) & 16.8 (9.6-24.0) & 12.5 (6.6-18.4) & 61.5 (58.9-64.0) & 28.9 (20.1-37.7) & 16.0 (10.3-21.7) \\
$2.5k$ & 98.8 (97.1-100) & 98.0 (95.2-100) & 98.0 (95.2-100 & 99.9 (99.7-100) & 100 (100-100) & 100 (100-100) \\
$5k$ & 98.9 (97.4-100) & 99.0 (97.0-100) & 98.2 (95.8-100) & 99.9 (99.7-100) & 100 (100-100) & 100 (100-100) \\
$10k$ & 99.7 (99.4-100) & 100 (100-100) & 99.2 (98.4-100) & 99.8 (99.5-100) & 100 (100-100) & 99.5 (98.5-100) \\
    \toprule
%%%%%%%%%%%%%%%%%%%%%
%% B1 unobserved
%%%%%%%%%%%%%%%%%%%%%
          & \multicolumn{6}{c}{\fontfamily{cmr}\textsc{\textbf{$B_1$ Unobserved}}} \\
         \cmidrule(lr){2-7} 
         %%%
         & \multicolumn{3}{c}{\textsc{Bernoulli $|$ Linear}} & \multicolumn{3}{c}{\textsc{Hypergeometric $|$ Quadratic}} \\
         \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
          %%%
         $n$ & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} \\
         %%%
         \hline
$1k$ & 71.3 (68.3-74.3) & 36.0 (27.7-44.3) & 32.0 (24.5-39.5) & x & x & x \\
$2.5k$ & 100 (100-100) & 100 (100-100) & 100 (100-100) & x & x & x \\
$5k$ & 99.1 (98.0-100) & 98.0 (95.2-100) & 97.7 (94.8-100) & x & x & x \\
$10k$ & 99.9 (99.7-100) & 100 (100-100) & 99.7 (99.0-100) & x & x & x \\
    \toprule
%%%%%%%%%%%%%%%%%%%%%
%% B2 unobserved
%%%%%%%%%%%%%%%%%%%%%
          & \multicolumn{6}{c}{\fontfamily{cmr}\textsc{\textbf{$B_2$ Unobserved}}} \\
         \cmidrule(lr){2-7} 
         %%%
         & \multicolumn{3}{c}{\textsc{Bernoulli $|$ Linear}} & \multicolumn{3}{c}{\textsc{Hypergeometric $|$ Quadratic}} \\
         \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
          %%%
         $n$ & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} \\
         %%%
         \hline
$1k$ & 72.0 (68.9-75.1) & 38.2 (29.9-46.5) & 35.0 (27.4-42.6) & x & x & x \\
$2.5k$ & 99.2 (97.8-100) & 99.0 (97.0-100) & 99.0 (97.0-100) & x & x & x \\
$5k$ & 100 (100-100) & 100 (100-100) & 100 (100-100) & x & x & x \\
$10k$ & 99.5 (98.7-100) & 99.0 (97.0-100) & 99.0 (97.0-100) & x & x & x \\
    \toprule
%%%%%%%%%%%%%%%%%%%%%
%% B3 unobserved
%%%%%%%%%%%%%%%%%%%%%
          & \multicolumn{6}{c}{\fontfamily{cmr}\textsc{\textbf{$B_3$ Unobserved}}} \\
         \cmidrule(lr){2-7} 
         %%%
         & \multicolumn{3}{c}{\textsc{Bernoulli $|$ Linear}} & \multicolumn{3}{c}{\textsc{Hypergeometric $|$ Quadratic}} \\
         \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
          %%%
         $n$ & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} \\
         %%%
         \hline
$1k$ & 68.8 (67.7-69.9) & 46.5 (44.0-49.0) & 31.0 (29.3-32.7) & x & x & x \\
$2.5k$ & 71.0 (70.4-71.6) & 51.7 (50.7-52.7) & 36.7 (34.7-38.6) & x & x & x \\
$5k$ & 77.2 (76.3-78.1) & 62.3 (60.9-63.8) & 58.0 (55.1-60.9) & x & x & x \\
$10k$ & 80.0 (80.0-80.0) & 66.7 (66.7-66.7) & 66.7 (66.7-66.7) & x & x & x \\
$25k$ & 79.9 (79.7-80.1) & 66.7 (66.7-66.7) & 66.7 (66.7-66.7) & x & x & x \\
     %%%%%%%%%%%%%%%%%%%
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Performance of Algorithm \ref{alg:method} on thirteen-node DAGs containing a butterfly structure (Figure \ref{fig:m_butterfly}) across noise distributions, causal mechanisms, and sample sizes ($n$). In all DAGs, exposure $X$ is a direct cause of outcome $Y$. Metrics reported are accuracy of all labels ($\z$ \textsc{Acc}), mean precision for partition $\z_1$ ($\z_1$ \textsc{Pre}), and mean recall for partition $\z_1$ ($\z_1$ \textsc{Rec}). The 95\% confidence interval over the 100 individual DAG metrics is reported in parentheses. Independence was determined by chi-square independence testing with $\alpha = 0.001$.} %{\color{red} Butterfly manual threshold = 0.01, 0.0075 for linear-hypergeometric}}
    \label{tab:results_butterfly}
\end{table}

==> tables_tex/table_m_butterfly_mi.tex <==
\begin{table}[!h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l ccc ccc}
    \toprule
        %%%%%%%%%%%%%%%%%%%%%
    %% M
    %%%%%%%%%%%%%%%%%%%%%
    & \multicolumn{6}{c}{\fontfamily{cmr}\textsc{\textbf{All variables observed}}} \\
    \cmidrule(lr){2-7} 
    %%%
     & \multicolumn{3}{c}{\textsc{Bernoulli $|$ Linear}} & \multicolumn{3}{c}{\textsc{Hypergeometric $|$ Quadratic}} \\
     \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
     %%%
$n$ & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} \\
\hline

$100$ & 40.5 (38.8-42.1) & 3.0 (0-6.4) & 42.9 (41.3-44.4) & 38.3 (36.8-39.8) & 0.0 (0.0-0.0) & 0.0 (0.0-0.0) \\
$500$ & 80.4 (77.7-83.1) & 81.0 (73.3-88.7) & 89.0 (81.2-96.8) & 50.6 (49.1-52.2) & 7.0 (2.0-12.0) & 50.0 (47.5-52.5) \\
$1k$ & 98.9 (98.3-99.5) & 100 (100-100) & 100 (100-100) & 88.4 (86.5-90.3) & 78.0 (69.8-86.2) & 77.2 (69.2-85.2) \\
%$2.5k$ & 100 (100-100) & 100 (100-100) & 100 (100-100) & 99.4 (98.9-99.8) & 100 (100-100) & 100 (100-100) \\
$5k$ & 100 (100-100) & 100 (100-100) & 100 (100-100) & 100 (100-100) & 100 (100-100) & 100 (100-100) \\
%$7.5k$ & 100 (100-100) & 100 (100-100) & 100 (100-100) & 100 (100-100) & 100 (100-100) & 100 (100-100) \\
%$10k$ & 100 (100-100) & 100 (100-100) & 100 (100-100) & 100 (100-100) & 100 (100-100) & 100 (100-100) \\
     %%%%%%%%%%%%%%%%%%%
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Performance of Algorithm \ref{alg:method} on thirteen-node DAGs containing an M-structure structure (Figure \ref{fig:m_butterfly}) across noise distributions, causal mechanisms, and sample sizes ($n$). In all DAGs, exposure $X$ is a direct cause of outcome $Y$. Metrics reported are accuracy of all labels ($\z$ \textsc{Acc}), precision for partition $\z_1$ ($\z_1$ \textsc{Pre}), and recall for partition $\z_1$ ($\z_1$ \textsc{Rec}). The 95\% confidence interval over the 100 individual DAG metrics is reported in parentheses. A heuristic independence threshold of 0.05 was used for all data generating processes.} %{\color{red} Butterfly manual threshold = 0.01, 0.0075 for linear-hypergeometric}}
    \label{tab:results_m_butterfly}
\end{table}


\begin{table}[!h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l ccc ccc}
    \toprule
%%%%%%%%%%%%%%%%%%%%%
%% BUTTERFLY
%%%%%%%%%%%%%%%%%%%%%
          & \multicolumn{6}{c}{\fontfamily{cmr}\textsc{\textbf{DAG with Butterfly Structure}}} \\
         \cmidrule(lr){2-7} 
         %%%
         & \multicolumn{3}{c}{\textsc{Bernoulli $|$ Linear}} & \multicolumn{3}{c}{\textsc{Hypergeometric $|$ Quadratic}} \\
         \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
          %%%
         $n$ & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} & \textsc{$\z$ Acc} & \textsc{$\z_1$ Prec} & \textsc{$\z_1$ Rec} \\
         %%%
         \hline
$1k$ & 42.0 (41.1-42.9) & 24.8 (24.3-25.2) & 50.0 (49.0-51.0) & 27.5 (27.2-27.7) & 0.0 (0.0-0.0) & 0.0 (0.0-0.0) \\
$1.5k$ & 48.7 (47.8-49.6) & 25.0 (25.0-25.0) & 50.0 (50.0-50.0) & 46.1 (43.0-49.2) & 10.5 (6.5-14.5) & 66.7 (61.3-72.0) \\
$2k$ & 71.7 (67.6-75.8) & 51.2 (44.2-58.3) & 75.9 (71.2-80.6) & 67.1 (65.3-68.9) & 34.5 (29.7-39.3) & 67.3 (61.1-73.5) \\
$2.5k$ & 94.5 (92.3-96.6) & 90.0 (86.1-93.9) & 94.7 (92.1-97.4) & 76.1 (73.4-78.8) & 53.5 (47.8-59.2) & 77.3 (71.4-83.1) \\
$5k$ & 100 (100-100) & 100 (100-100) & 100 (100-100) & 97.3 (96.1-98.5) & 93.5 (90.9-96.1)  & 98.9 (97.7-100) \\
%$7.5k$ & 100 (100-100) & 100 (100-100) & 100 (100-100) & 98.8 (98.2-99.4) & 96.8 (95.1-98.4)  & 100 (100-100) \\
$10k$ & 100 (100-100) & 100 (100-100) & 100 (100-100) & 99.2 (98.7-99.7) & 97.8 (96.3-99.2) & 100 (100-100) \\
     %%%%%%%%%%%%%%%%%%%
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Performance of Algorithm \ref{alg:method} on thirteen-node DAGs containing a butterfly structure (Figure \ref{fig:m_butterfly}) across noise distributions, causal mechanisms, and sample sizes ($n$). In all DAGs, exposure $X$ is a direct cause of outcome $Y$. Metrics reported are accuracy of all labels ($\z$ \textsc{Acc}), precision for partition $\z_1$ ($\z_1$ \textsc{Pre}), and recall for partition $\z_1$ ($\z_1$ \textsc{Rec}). The 95\% confidence interval over the 100 individual DAG metrics is reported in parentheses. A heuristic independence threshold of 0.05 was used for all data generating processes.} %{\color{red} Butterfly manual threshold = 0.01, 0.0075 for linear-hypergeometric}}
    \label{tab:results_butterfly}
\end{table}

==> tables_tex/table_motivation.tex <==
\begin{table}[!ht]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lcccccc}
    \toprule
        ~ & \multicolumn{2}{c}{\fontfamily{cmr}\textsc{\textbf{Percent Valid}}} & \multicolumn{2}{c}{\fontfamily{cmr}\textsc{\textbf{Mean Runtime}}} & \multicolumn{2}{c}{\fontfamily{cmr}\textsc{\textbf{Mean total tests}}} \\ 
        n & LDP & PC & LDP & PC & LDP & PC \\ 
        1k & 36.0 & 0 & 0.012 (0.01-0.013) & 0.169 (0.155-0.182) & 50.5 (48.9-52.1) & 232.3 (215.9-248.7) \\ 
        2.5k & 68.0 & 0 & 0.012 (0.011-0.014) & 0.224 (0.211-0.237) & 58.4 (56.286-60.514) & 281.04 (275.282-286.798) \\ 
        5k & 96.0 & 0 & 0.013 (0.011-0.014) & 0.258 (0.249-0.267) & 61.56 (60.698-62.422) & 283.88 (281.591-286.169) \\ 
        7.5k & 100 & 0 & 0.013 (0.011-0.014) & 0.29 (0.282-0.298) & 62.0 (62.0-62.0) & 287.08 (284.46-289.7) \\ 
        10k & 100 & 0 & 0.012 (0.011-0.013) & 0.331 (0.312-0.35) & 62.0 (62.0-62.0) & 292.16 (287.083-297.237) \\ 
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{}
    \label{tab:motive}
\end{table}

==> tables_tex/table_motive.tex <==
\begin{table}[!t]
    \centering
    \begin{adjustbox}{max width=0.45\textwidth}
    \begin{tabular}{c c c c c}
    \toprule
        \textsc{True Graph} & & \multicolumn{3}{c}{\textsc{Causal Partition}} \\
         %%%%
         \cmidrule(lr){3-5}
         %%%
         \multirow{9}{*}{\fbox{\begin{tabular}{@{}c@{}}
        \includegraphics[height=0.1\textheight]{figures/motive_ground_truth.png} \\
        \tiny Exposure-outcome pair $\{X,Y\}$. \vspace{-1mm} \\ 
        \tiny Confounders (partition $\z_1$) in red. \vspace{-1mm}  \\ \tiny Instruments (partition $\z_5$) in green.
        \end{tabular}}} & \textsc{Node} & \textsc{True} & \textsc{PC} & \textsc{LDP}  \\
        %%%
        \cmidrule(lr){2-5}
         & $Z_1$ & $\z_1$ & $\z_8$ \xmark & $\z_1$ \cmark \\
        & $B_1$ & $\z_1$ & $\z_1$ \cmark & $\z_1$ \cmark \\
        & $B_2$ & $\z_1$ & $\z_1$ \cmark & $\z_1$ \cmark \\
        & $B_3$ & $\z_1$ & $\z_1$ \cmark & $\z_1$ \cmark \\
        & $Z_4$ & $\z_4$ & $\z_4$ \cmark & $\z_4$ \cmark \\
        & $Z_5$ & $\z_5$ & $\z_1$ \xmark & $\z_5$ \cmark \\
        & $Z_7$ & $\z_7$ & $\z_7$ \cmark & $\z_7$ \cmark \\
        & $Z_8$ & $\z_8$ & $\z_8$ \cmark & $\z_8$ \cmark \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{LDP is motivated by failure modes of global causal discovery under finite samples. For sample sizes $n \leq 10k$, classic constraint-based algorithm PC \citep{spirtes_causation_2000} cannot infer the correct causal partitions of $\z$. While PC consistently mislabels instrument $Z_5$ and confounder $Z_1$, LDP correctly identifies instruments and valid adjustment sets for $\{X,Y\}$ with fewer tests, smaller samples, and faster runtimes (Figure \ref{fig:motive_times_tests}). Additional details and results for PC and FCI in Appendix \ref{sec:global}.}
    \label{tab:motive}
\end{table}


==> tables_tex/table_notation.tex <==
\begin{table}[!h]
    \centering
    \begin{adjustbox}{max width=0.47\textwidth}
    \begin{tabular}{l l l}
        \toprule
        \textsc{Notation} & \textsc{Properties} & \textsc{Meaning} \\
        \hline
        %%%
        $\{X,Y\}$ & $X \in \mathbb{R}^{n}$, $Y \in \mathbb{R}^{n}$ & Exposure and outcome. \\
        %%%
        $\mathbf{Z}$ & $\mathbf{Z} \in \mathbb{R}^{n \times m}$ & Background set of variables. \\
        %%%
        $Z$ & $Z \in \mathbf{Z}$ & Candidate of unknown type. \\
        %%%
        $\g$ & $X \cup Y \cup \mathbf{Z} \in \mathcal{G}_{XY\mathbf{Z}}$ & Graph induced by $\{X,Y,\mathbf{Z}\}$. \\ %\\
        %%%
        %\underline{\textsc{Subsets of} $\mathbf{Z}$} \\
        %\textsc{Subsets of} $\mathbf{Z}$ \\
        %\hline
        %%%
        %$\mathbf{Z}_1$ & $Z_1 \in \mathbf{Z}_1$, $|\mathbf{Z}_1| \geq 0$ & All confounders for $\{X,Y\}$. \\
        %%%
        %$\mathbf{Z}_2$ & $Z_2 \in \mathbf{Z}_2$, $|\mathbf{Z}_2| \geq 0$ & All colliders for $\{X,Y\}$. \\
        %%%
        %$\mathbf{Z}_3$ & $Z_3 \in \mathbf{Z}_3$, $|\mathbf{Z}_3| \geq 0$ & All mediators for $\{X,Y\}$. \\
        %%%
        %$\mathbf{Z}_4$ & $Z_4 \in \mathbf{Z}_4$, $|\mathbf{Z}_4| \geq 1$ & All causes of $Y$. \\
        %%%
        %$\mathbf{Z}_5$ & $Z_5 \in \mathbf{Z}_5$, $|\mathbf{Z}_5| \geq 1$ & All causes of $X$. \\
        %%%
        %$\mathbf{Z}_6$ & $Z_6 \in \mathbf{Z}_6$, $|\mathbf{Z}_6| \geq 0$ & All effects of $Y$. \\
        %%%
        %$\mathbf{Z}_7$ & $Z_7 \in \mathbf{Z}_7$, $|\mathbf{Z}_7| \geq 0$ & All effects of $X$. \\
        %%%
        %$\mathbf{Z}_8$ & $Z_8 \in \mathbf{Z}_8$, $|\mathbf{Z}_8| \geq 0$ & All isolated from $\{X,Y\}$. \\
    \toprule
    \end{tabular}
    \end{adjustbox}
    \caption{Notation referenced throughout. Partitions of $\z$ are defined in Table \ref{tab:partitions}.}
    \label{tab:vars}
\end{table}

==> tables_tex/table_old_mildew.tex <==
\begin{table}[!h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l cccc cccc cccc}
        \toprule[1pt]
        %%%
        &  \multicolumn{12}{c}{\fontfamily{cmr}\textsc{\textbf{Mildew}}  \textsc{mikro\_1} $\to$ \textsc{meldug\_2} ($|\z| = 14$, $|\z_1| = 2$)} \\
        \cmidrule(lr){2-13}
        %%%
         &  \multicolumn{4}{c}{\textsc{Algorithm \ref{alg:method}}} &  \multicolumn{4}{c}{\textsc{PC}} & \multicolumn{4}{c}{\textsc{FCI}}  \\ 
         %%%
         \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
         %%%
         $n$ & $\z$ \textsc{Acc} & $\z_1$ \textsc{Pre} & $\z_1$ \textsc{Rec} & \cmark & $\z$ \textsc{Acc} & $\z_1$ \textsc{Pre} & $\z_1$ \textsc{Rec} & \cmark & $\z$ \textsc{Acc} & $\z_1$ \textsc{Pre} & $\z_1$ \textsc{Rec} & \cmark \\
         %%%
         \hline
         %%%
         $10k$ & 71.4 (54.3-88.6) & 46.7 (2.4-91.0) & 50.0 (6.2-93.8) & x & x & x & x & x & x & x  & x & x \\
         $25k$ & 92.9 (88.4-97.3) & 93.3 (80.3-100) & 100 (100-100) & x & x & x & x & x & x & x  & x & x \\
         $50k$ & 97.1 (93.7-100) & 100 (100-100) & 100 (100-100) & x & x & x & x & x & x & x  & x & x \\
         %$100k$ & x & x & x & x & x & x & x & x & x & x  & x & x \\
         %%%
         \bottomrule[1pt]
    \end{tabular}
    \end{adjustbox}
    \caption{Performance of Algorithm \ref{alg:method} on the subsetted \textsc{Mildew} benchmark from \texttt{bnlearn} \citep{scutari_learning_2010}, with \textsc{mikro\_1} as exposure and \textsc{meldug\_2} as outcome. While the original DAG contains 35 nodes, a subset of 14 nodes and the exposure-outcome pair were submitted to Algorithm \ref{alg:method}. Independence was determined by chi-square independence testing with $\alpha = 0.005$. All values are averaged over five independent data samples from the ground truth DAG, with 95\% confidence intervals in parentheses. Sample size is denoted by $n$. Metrics reported are mean accuracy of all labels ($\z$ \textsc{Acc}), mean precision for partition $\z_1$ ($\z_1$ \textsc{Pre}), mean recall for partition $\z_1$ ($\z_1$ \textsc{Rec}), and fraction of replicates that admit a sufficient adjustment set (\cmark). }
    \label{tab:mildew2} 
\end{table}

==> tables_tex/table_paths.tex <==
\newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}

\begin{table}[!h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l l l}
    \toprule[1pt]
        \textsc{Type} & \textsc{Active Path Relative to $X$} & \textsc{Active Path Relative to $Y$} \\
        \hline
        %%%
        1 & None (or none that do not pass through $Y$). & None (or none that do not pass through $X$). \\
        2 & $Z \rightarrow \dots \rightarrow X$ path(s) and no other types. & $Z \rightarrow \dots \rightarrow Y$ path(s) not passing through $X$ and no other types. \\
        3 & $X \rightarrow \dots \rightarrow Z$ path(s) not passing through $Y$ and no other types. & $Y \rightarrow \dots \rightarrow Z$ path(s) and no other types. \\
        4 & $Z \leftarrow \dots Z' \dots \rightarrow X$ path(s) and no other types. & $Z \leftarrow \dots Z' \dots \rightarrow Y$ path(s) and no other types. \\
        5 & Type 2 path(s) and Type 4 path(s). & Type 2 path(s) and Type 4 path(s). \\
        6 & Type 3 path(s) and Type 4 path(s). & Type 3 path(s) and Type 4 path(s). \\
    \bottomrule[1pt]
    \end{tabular}
    \end{adjustbox}
    \caption{Exhaustive enumeration of the types of active paths that can lie between any given $Z$ and $\{X,Y\}$. In confounded paths, $Z'$ denotes an additional variable in $\z$ that may or may not belong to the same partition as $Z$. Note that Type 1 and Type 2 paths cannot coincide for a single $Z$, as this would induce a cycle.}
    \label{tab:path_types}
\end{table}

\begin{table}[!h]
    \centering
    \begin{tabular}{c | c || c c c c c c}
        \toprule
        \multicolumn{2}{c}{} & \multicolumn{6}{c}{\textsc{Relative to $X$}} \\
        \cmidrule(lr){3-8}
         \multicolumn{2}{c}{} & \textsc{Type 1} & \textsc{Type 2} & \textsc{Type 3} & \textsc{Type 4} & \textsc{Type 5} & \textsc{Type 6} \\
         \hline 
         \hline
         \vspace{-1.8mm}
         %\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textsc{Relative to $Y$}}}} & & & & & & & \\
         \multirow{6}{*}{\STAB{\rotatebox[origin=c]{90}{\textsc{Relative to $Y$ }}}} & & & & & & & \\
         & \textsc{Type 1} & $\z_8$ & $\z_5$ & $\z_7$ & $\z_5$ & $\z_5$ & $\z_7$ \\
         & \textsc{Type 2} & $\z_4$ & $\z_1$ & $\z_3$ & $\z_1$ & $\z_1$ & $\z_3$ \\
         & \textsc{Type 3} & $\z_6$ & $\emptyset$ & $\z_2$ & $\z_2$ & $\emptyset$ & $\z_2$ \\
         & \textsc{Type 4} & $\z_4$ & $\z_1$ & $\z_2$ & $\z_{2 \in \mathbf{M}_3}$ & $\z_1$ & $\z_2$ \\
         & \textsc{Type 5} & $\z_4$ & $\z_1$ & $\z_3$ & $\z_1$ & $\z_{1 \in \mathbf{B}_3}$ & $\z_3$ \\
         & \textsc{Type 6} & $\z_6$ & $\emptyset$ & $\z_2$ & $\z_2$ & $\emptyset$ & $\z_2$\\
         \bottomrule
    \end{tabular}
    \caption{Combinations of active path types relative to $X$ and $Y$. Cells contain partitions that can participate in the given combination of active path types. The empty set ($\emptyset$) indicates that this combination of active path types is forbidden under the acyclicity constraint. A subscript of $\mathbf{M}_3$ indicates that this variable is an M-collider, while a subscript of $\mathbf{B}_3$ denotes a butterfly-type confounder (Figure \ref{fig:m_butterfly}).}
    \label{tab:path_grid}
\end{table}



==> tables_tex/table_simple_secondary.tex <==
\begin{table*}[!h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l c c c c c c}
    %%%%%%%%%%%%%%%%%%%%%
    % BERNOULLI
    %%%%%%%%%%%%%%%%%%%%%
    \toprule[1pt]
         & \multicolumn{6}{c}{\fontfamily{cmr}\textsc{\textbf{Bernoulli Noise}}}  \\ 
         %%%
        \cmidrule(lr){2-7} 
        %%%
         & \multicolumn{2}{c}{\textsc{Linear}} & \multicolumn{2}{c}{\textsc{Quadratic}} & \multicolumn{2}{c}{\textsc{Cube Root}} \\
         %%%
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
        %%%
        \textsc{Sample Size} & \textsc{$X \to Y$} & \textsc{$X \not\to Y$} & \textsc{$X \to Y$} & \textsc{$X \not\to Y$} & \textsc{$X \to Y$} & \textsc{$X \not\to Y$} \\
        %%%
        \hline
         $n = 100$ & 46.88 (19.31) & x & 41.13 (13.50) & 39.88 (14.65) & 41.63 (16.49) & 29.38 (15.25) \\
         $n = 500$ & 90.75 (15.67) & x & 68.63 (14.09) & 72.13 (12.61) & 74.50 (4.98) & 66.13 (8.89)  \\
         $n = 1k$ & 94.13 (13.52) & x & 79.38 (11.91) & 79.63 (13.54) & 78.38 (9.16) & 74.88 (3.31) \\
         $n = 5k$ & 96.50 (11.19) & x & 96.88 (9.58) & 98.00 (8.05) & 98.88 (3.58) & 88.75 (12.44)  \\
         $n = 10k$ & 97.38 (9.07) & x & 99.63 (3.73) & 94.50 (13.15) & 99.00 (3.39) & 94.00 (10.68) \\
         $n = 50k$ & 97.88 (8.49) & x & 99.63 (3.73) & 98.13 (8.17) & 98.75 (3.75) & 93.50 (10.97) \\
         $n = 100k$ & 96.63 (11.97) & x & 100.0 (0.0) & 96.75 (10.40) & 99.00 (3.39) & 94.25 (10.52)  \\
    \toprule[1pt]
    %%%%%%%%%%%%%%%%%%%%%
    % HYPERGEOMETRIC
    %%%%%%%%%%%%%%%%%%%%%
    & \multicolumn{6}{c}{\fontfamily{cmr}\textsc{\textbf{Hypergeometric Noise}}} \\ 
         %%%
        \cmidrule(lr){2-7} 
        %%%
         & \multicolumn{2}{c}{\textsc{Linear}} & \multicolumn{2}{c}{\textsc{Quadratic}} & \multicolumn{2}{c}{\textsc{Cube Root}} \\
         %%%
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
        %%%
        \textsc{Sample Size} & \textsc{$X \to Y$} & \textsc{$X \not\to Y$} & \textsc{$X \to Y$} & \textsc{$X \not\to Y$} & \textsc{$X \to Y$} & \textsc{$X \not\to Y$} \\
        %%%
        \hline
         $n = 100$ & 48.63 (19.28) & x & 35.75 (14.14) & 39.50 (12.84) & 38.00 (15.10) & x \\
         $n = 500$ & 91.63 (16.01) & x & 65.13 (10.35) & 71.00 (12.23) & 74.63 (3.73) & x \\
         $n = 1k$ & 96.13 (11.14) & x & 80.25 (11.07) & 81.25 (12.44) & 78.75 (8.98) & x \\
         $n = 5k$ & 99.63 (3.73) & x & 100.0 (0.0) & 100.0 (0.0) & 99.75 (2.49) & x \\
         $n = 10k$ & 98.75 (6.25) & x & 100.0 (0.0) & 99.63 (3.73) & 100.0 (0.0) & x \\
         $n = 50k$ & 98.38 (7.21) & x & 100.0 (0.0) & 100.0 (0.0) & 100.0 (0.0) & x \\
         $n = 100k$ & 97.38 (10.05) & x & 100.0 (0.0) & 100.0 (0.0) & 100.0 (0.0) & x \\
    \toprule[1pt]
    %%%%%%%%%%%%%%%%%%%%%
    % UNIFORM
    %%%%%%%%%%%%%%%%%%%%%
    & \multicolumn{6}{c}{\fontfamily{cmr}\textsc{\textbf{Uniform Noise}}} \\
         %%%
        \cmidrule(lr){2-7} 
        %%%
         & \multicolumn{2}{c}{\textsc{Linear}} & \multicolumn{2}{c}{\textsc{Quadratic}} & \multicolumn{2}{c}{\textsc{Cubic}} \\
         %%%
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
        %%%
        \textsc{Sample Size} & \textsc{$X \to Y$} & \textsc{$X \not\to Y$} & \textsc{$X \to Y$} & \textsc{$X \not\to Y$} & \textsc{$X \to Y$} & \textsc{$X \not\to Y$} \\
        %%%
        \hline
         $n = 100$ & 42.13 (18.08) & x & x & x & x & x \\
         $n = 500$ & 59.63 (19.99) & x & x & x & x & x \\
         $n = 1k$ & 69.88 (18.29) & x & x & x & x & x \\
         $n = 5k$ & 88.75 (15.56) & x & x & x & x & x \\
         $n = 10k$ & 89.75 (14.62) & x & x & x & x & x \\
         $n = 50k$ & x & x & x & x & x & x \\
         $n = 100k$ & x & x & x & x & x & x \\
    \toprule[1pt]
    %%%%%%%%%%%%%%%%%%%%%
    % EXPONENTIAL
    %%%%%%%%%%%%%%%%%%%%%
    & \multicolumn{6}{c}{\fontfamily{cmr}\textsc{\textbf{Exponential Noise}}} \\
         %%%
        \cmidrule(lr){2-7} 
        %%%
         & \multicolumn{2}{c}{\textsc{Linear}} & \multicolumn{2}{c}{\textsc{Quadratic}} & \multicolumn{2}{c}{\textsc{Cubic}} \\
         %%%
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
        %%%
        \textsc{Sample Size} & \textsc{$X \to Y$} & \textsc{$X \not\to Y$} & \textsc{$X \to Y$} & \textsc{$X \not\to Y$} & \textsc{$X \to Y$} & \textsc{$X \not\to Y$} \\
        %%%
        \hline
         $n = 100$ & x & x & x & x & x & x \\
         $n = 500$ & x & x & x & x & x & x \\
         $n = 1k$ & x & x & x & x & x & x \\
         $n = 5k$ & x & x & x & x & x & x \\
         $n = 10k$ & x & x & x & x & x & x \\
         $n = 50k$ & x & x & x & x & x & x \\
         $n = 100k$ & x & x & x & x & x & x \\
    \toprule[1pt]
    \end{tabular}
    \end{adjustbox}
    \caption{Accuracy of Algorithm \ref{alg:method} on a simple ten-node DAG (Figure \ref{fig:ten_node_dag}) across noise distributions, causal mechanisms, and sample sizes ($n$). All DAGs feature one node per partition ($\z_1 - \z_8$). Reported values are averaged over 100 DAGs (i.e. 800 variables total, excluding all exposure-outcome pairs). The standard deviation over single-DAG accuracies is reported in parentheses. Data generating processes where $X$ is a direct cause of $Y$ are denoted by $X \to Y$, with $X \not\to Y$ denoting no direct causal effect of $X$ on $Y$. Hyperparameter values are reported in the appendix.} %{\color{red} manual threshold = 0.03 for all $X \to Y$. For $X \not\to Y$: Bernoulli cube root manual threshold = 0.015, all others 0.03.}}
    \label{tab:results_ten_node_dag}
\end{table*}


\begin{table}[!h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l c c c c c c c c}
    \toprule
         & \multicolumn{4}{c}{\fontfamily{cmr}\textsc{\textbf{M-Structure}}} & \multicolumn{4}{c}{\fontfamily{cmr}\textsc{\textbf{Butterfly Structure}}} \\
         \cmidrule(lr){2-5} \cmidrule(lr){6-9}
         %%%
          & \multicolumn{2}{c}\textsc{Bernoulli $|$ Quadratic} & \multicolumn{2}{c}\textsc{Hypergeometric $|$ Quadratic} & \multicolumn{2}{c}\textsc{Bernoulli $|$ Quadratic} & \multicolumn{2}{c}\textsc{Hypergeometric $|$ Quadratic} \\
          \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} 
          %%%
         \textsc{Sample Size} & \textsc{$X \to Y$} & \textsc{$X \not\to Y$} & \textsc{$X \to Y$} & \textsc{$X \not\to Y$} & \textsc{$X \to Y$} & \textsc{$X \not\to Y$} & \textsc{$X \to Y$} & \textsc{$X \not\to Y$} \\
         %%%
         \hline
         $n = 1k$ & x & x & x & x & x & x & x & 35.18 (4.75)  \\
         $n = 5k$ & x & x & x & x & x & 42.18 (7.33) & x & 42.45 (7.05)  \\ 
         $n = 10k$ & x & x & x & x & x & 70.82 (17.78) & x & 66.09 (13.72)  \\
         $n = 25k$ & x & x & x & x & x & 88.82 (14.31) & 86.36 (17.60) & 88.73 (14.89)  \\
         $n = 50k$ & x & x & x & 90.91 (0.0) & x & 100.0 (0.0) & 100.0 (0.0) & 100.0 (0.0)  \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Accuracy of Algorithm \ref{alg:method} on ten-node DAGs with an additional M-structure or butterfly structure (Figure \ref{fig:m_butterfly}).} %{\color{red} Butterfly manual threshold = 0.01}}
    \label{tab:results_m_butterfly}
\end{table}
